Local scale invariance and robustness of proper scoring rules

Averages of proper scoring rules are often used to rank probabilistic forecasts. In many cases, the individual terms in these averages are based on observations and forecasts from different distributions. We show that some of the most popular proper scoring rules, such as the continuous ranked probability score (CRPS), give more importance to observations with large uncertainty which can lead to unintuitive rankings. To describe this issue, we define the concept of local scale invariance for scoring rules. A new class of generalized proper kernel scoring rules is derived and as a member of this class we propose the scaled CRPS (SCRPS). This new proper scoring rule is locally scale invariant and therefore works in the case of varying uncertainty. Like CRPS it is computationally available for output from ensemble forecasts, and does not require the ability to evaluate densities of forecasts. We further define robustness of scoring rules, show why this also is an important concept for average scores, and derive new proper scoring rules that are robust against outliers. The theoretical findings are illustrated in three different applications from spatial statistics, stochastic volatility models, and regression for count data.

==> probpred_text.tex <==
\section{Introduction}
A popular way of assessing the goodness-of-fit of statistical models is to quantify their predictive ability. 
This is often done by evaluating the accuracy of point predictions, using for example mean-squared errors between the predictions and the observed data. However, one is typically also interested in the ability to correctly quantify the prediction uncertainty. 
%
To fully quantify the prediction uncertainty one must use the model's entire predictive distribution, which often is referred to as probabilistic forecasting \citep{gneiting2007probabilistic}. The main method for summarizing the accuracy of probabilistic forecasts is to use averages of proper scoring rules.

A scoring rule $S(\P,y)$ is a real-valued function of a probability measure $\P$ that represents the forecast or prediction and the observed outcome $y$. We use $S(\P,\Q)$ to denote the expected value of $S(\P,y)$ when $y \sim \Q$. The scoring rule is said to be proper if $S(\Q,\Q) \geq S(\P,\Q)$, and strictly proper if equality holds if and only if $\P=\Q$ \citep{gneiting2007strictly}. Using a strictly proper scoring rule for model selection has the desirable property that the best model is always the true distribution $\Q$ in the long run. This can be seen as keeping the forecaster earnest, in the sense that he or she should always use the estimate of the probability distribution that is being predicted to get the best expected score.

The two most popular proper scoring rules are the log-score and the continuous ranked probability score (CRPS). Variants of the two scores have been used in several different fields of research and applications, such as electricity price forecasting \citep{nowotarski2018recent}, wind speed modeling \citep{baran2016mixture,lerch2013comparison}, weather forecasting \citep{brocker2012evaluating}, financial prediction \citep{opschoor2017combining}, precipitation modeling \citep{ingebrigtsen2015estimation}, and spatial statistics \citep{fuglstad2015does}. The log-score is defined as 
$\logs(\P,y) = \log f(y)$, and the CRPS is defined as
\begin{align*}
\crps(\P,y) &= - \int (F(x) - 1(x\geq y))^2 dx = \frac1{2}\pE_{\P,\P}[|X-Y|] - \pE_{\P}[|X-y|],
\end{align*}
where $f(\cdot)$ and $F(\cdot)$ respectively denote the density and cumulative distribution functions corresponding to $\P$ \citep{gneiting2007strictly}. Here and in what follows, we use the notation $\E_{\P}[g(X)]$ for the expected value of a function $g(X)$ of a random variable $X$ with distribution $\P$. Furthermore, $\E_{\P,\Q}[g(X,Y)]$ denotes the expected value of $g(X,Y)$ when $X\sim\P$ and $Y\sim\Q$ are independent. 

The predictive ability of a model for a set of observations $\{y_i\}_{i=1}^n$ is typically assessed using an average score 
\begin{equation}\label{eq:average_score}
S_n = \frac1{n}\sum_{i=1}^n S(\P_{i},y_i),
\end{equation}
where $\P_{i}$ denotes the predictive distribution for $y_i$ based on the model. These different predictive distributions might, for example, be one-step ahead predictions in a time series model or leave-one-out cross-validation predictions for a model in spatial statistics. 
%
The use of average scores for model comparison is natural, but we will show that it may lead to unintuitive model rankings if popular scoring rules such as the CRPS are used. There are two main reasons for this: Firstly, there is always some degree of model miss-specification for the models that are compared, and one model is rarely  best for all different observations. Secondly, the predictive distributions are typically different for the observations, and depending on the scoring rule that is used, each observation may therefore not be equally important for the average score. 

A situation where the latter problem occurs is when the different observations have varying degrees of predictability, like when the variances of the predictive distributions are different. This for example occurs frequently for weather and climate data which have large spatial and temporal variability in their predictability \citep{campbell2005}.
A strategy for dealing with this in climate science has been to use so-called skill scores, which typically take the form
$$
\frac{S_n - S_n^{ref}}{S_n^{ref}} \quad \text{or} \quad \frac{S_n - S_n^{ref}}{S_n^{opt} - S_n^{ref}}.
$$
Here $S_n$ is the score by the forecaster and $S_n^{ref}$ is a score for a reference method \citep{Winkler1996}. In the second version, $S_n^{opt}$ is a hypothetical optimal forecast  \citep[][Chapter 7.1.4]{wilks2005}. This standardization may seem natural since the score equals $1$ for the optimal forecast, is positive whenever the forecaster is better than the reference, and negative otherwise. It could also solve the problem with varying predictability if this information is present in the reference method. However, skill scores are in general improper even if they are based on a proper scoring rule \citep{murphy1973, gneiting2007strictly}. 

In this work, we will define and analyze properties for average scoring rules in the case of varying predictability, by examining differently scaled observations and predictions. One of our main results is to propose a method for standardizing proper scoring rules in a way so that they remain proper. More specifically, the main contribution of this work is twofold:
\begin{enumerate}
\item[(i)] We introduce two properties of scoring rules which are important if the average scores are used for model selection: Local scale invariance and robustness. We show that popular scoring rules such as the CRPS, root mean square error, and mean absolute error lack both of these properties and illustrate why this is a problem through several examples and three different applications in spatial statistics, regression modeling, and finance. 
\item[(ii)] We propose a new class of proper scoring rules that maintain the good properties of the CRPS, such as easy-to-use expressions that facilitate straight-forward Monte Carlo approximations of the scores in cases when the density of the model is unknown. Among these new proper scoring rules, we show that there are some special cases which are scale invariant and some that are robust, which solves the problems encountered in the above-mentioned applications.
\end{enumerate}
An example of a new scoring rule is the scaled CRPS, or SCRPS, which we define as 
\begin{equation}\label{eq:scrps}
\scrps(\P, y) := - \frac{\E_{\P}\left[ |X-y| \right]}{\E_{\P,\P}\left[ |X-Y| \right]} - \frac{1}{2}\log\left( \E_{\P,\P}\left[ |X-Y| \right]\right).
\end{equation}
Compared to CRPS, the SCRPS has the desirable property that the penalty of an incorrect prediction, $\E_{\P}\left[ |X-y| \right]$, is standardized by $\E_{\P,\P}\left[ |X-Y| \right]$. So for instance if the prediction expects a large uncertainty, then the penalty of making a large error is down-weighted. This is a fundamental property for being locally scale invariant, which we show that the SCRPS is. 

The structure of the article is as follows.  In the next section, we introduce the concepts of local scale invariance and robustness for scoring rules, and provide illustrative examples of why the lack of these properties may lead to unintuitive conclusions for model selection. In Section~\ref{sec:kernel_scores}, we analyze the class of kernel scores, which contains the CRPS as a special case, in terms of robustness and scale invariance. In the section, we also propose a robust version of the CRPS. 
%
Section~\ref{sec:standardized_scores} introduces a new general family of scoring rules, of which the SCRPS is a special case. We analyze these scores in terms of local scale invariance and robustness. Section~\ref{sec:application} presents three different applications where we illustrate the benefits of the new scoring rules. The article concludes with a discussion in Section~\ref{sec:discussion}. The article contains two appendices with (A) formulas for the new scoring rules for Gaussian distributions, and (B) a characterization of scoring rules in terms of generalized entropy. The supplementary materials contain all proofs.

%The supplementary materials of the article contains three appendices that (A) provides formulas for the new scoring rules for Gaussian distributions, (B) presents a characterization of scoring rules in terms of generalized entropy,  and (C) contains all proofs. 

\section{Local scale invariance and robustness of scoring rules}\label{sec:properties}
%In this section, we define the concepts of scale invariance and robustness of scoring rules. These will be used to better understand the behavior of commonly used scoring rules, and serve as a motivation for the new scoring rules that we later propose.

\subsection{Local scale invariance}\label{sec:scale}
As previously mentioned, the predictive measures $\P_{i}$ in \eqref{eq:average_score} often have varying uncertainty. Two common causes for this is that one either has a non-stationary model or that the observation locations are irregularly spaced. The latter is especially common for geostatistical applications. In the case of varying uncertainty, the magnitude of the value given by the scoring rule at each location can be dependent on the magnitude of this uncertainty. This is what we will refer to as scale dependence, or the lack of scale invariance. 

If the average score \eqref{eq:average_score} is used to compare the models, the scale dependence will make the different observations in the sum contribute differently to the average score. In other words, the weighting of the predictive ability for the different observations will depend on how the scoring rule depends on the uncertainty. This means that emphasis may be put on accurately predicting observations with certain scales, which can cause unintuitive results. 


 
\begin{example}\label{ex1}
Consider a situation with two observations $Y_i \sim \Q_{\theta_i}= \pN(0,\sigma_i^2), i=1,2,$ with $\sigma_1 = 0.1$ and $\sigma_2 = 1$. Assume that we want to evaluate a model which has predictive distributions  $\P_{i} = \pN(\hat{\mu}_i,\hat{\sigma}_i^2)$ for $Y_i$, using the average of a proper scoring rule for the two observations, $\frac12 S(\P_{1},Y_1) +\frac12 S(\P_{2},Y_2)$. Using the expressions in Appendix \ref{app:gauss}, we compute the expected average score when the CRPS, the SCRPS, and the log-score are used, and investigate how the average scores depend on the model parameters. The top row of Figure~\ref{fig:bivar} shows the result when varying the two standard deviations, $\hat{\sigma}_i$, while  $\hat{\mu}_i=0$. In the bottom row, the average scores are instead shown as functions of $\hat{\mu}_i$, while $\hat{\sigma}_i = \sigma_i$. To simplify interpretation, the scale of $\hat{\mu}_i$ is in quantile of the true distribution, i.e., $\hat{\mu}_i = \sigma_i\Phi^{-1}(q_i)$ where $q_i$ is the quantile. In both rows, one can note that the average CRPS is much more sensitive in relative errors in the second variable, which has the higher variance. Thus, if we would compare  two competing models for this example using CRPS, the model which has the better prediction for the second variable will likely win, even if it is much worse for the first variable.  As seen in the figure, this is not the case for the log-score and the SCRPS. 
\end{example}

\begin{figure}[!t]
	\begin{center}
		\begin{minipage}[t]{0.32\linewidth}
			\begin{center}
				CRPS\\
				%$\frac1{2}\sum_{i=1}^2\pE[CRPS(N(\mu_i,\hat{\sigma}_i),Y_i)]$\\
				\includegraphics[width=\textwidth]{bivariate_sigma_crps.png}\\
				\includegraphics[width=\textwidth]{bivariate_mu_crps.png}
			\end{center}
		\end{minipage}
		\begin{minipage}[t]{0.32\linewidth}
			\begin{center}
				log(LS)\\
				%$\frac1{2}\sum_{i=1}^2\pE[CRPS(N(\mu_i,\hat{\sigma}_i),Y_i)]$\\
				\includegraphics[width=\textwidth]{bivariate_sigma_logs.png}\\
				\includegraphics[width=\textwidth]{bivariate_mu_logs.png}
			\end{center}
		\end{minipage}
		\begin{minipage}[t]{0.32\linewidth}
			\begin{center}
				SCRPS\\
				%$\frac1{2}\sum_{i=1}^2\pE[CRPS(N(\mu_i,\hat{\sigma}_i),Y_i)]$\\
				\includegraphics[width=\textwidth]{bivariate_sigma_brps.png}\\
				\includegraphics[width=\textwidth]{bivariate_mu_brps.png}
			\end{center}
		\end{minipage}
		
	\end{center}
	\caption{Average expected CRPS, log-score, and SCRPS for two mean-zero normal distributions with $\sigma_1 = 0.1$ and $\sigma_2 = 1$. The top row shows the values as functions of the relative errors in the standard deviations of the predictive distributions when the predictive model has the correct mean value. The bottom row shows the values as functions of the quantiles $q_1$ and $q_2$, when the predictive model has correct variances but mean values $\hat{\mu}_i = \sigma_i\Phi^{-1}(q_i)$. }
	\label{fig:bivar}
\end{figure}


The example shows that, in the case of the normal distribution, CRPS and log-score have very different weighting of the observations due to the variable uncertainty (scaling) in the predictions. This has important implications for the case when the average scores are used to evaluate statistical models with dependence. For example, if different random field models for irregularly spaced observations are evaluated using leave-one-out cross validation, the predictive distributions for locations that are far away from other locations will have larger variances and thus be weighted higher when computing the average CRPS. It will therefore be most important to not have large errors for observations without any close neighbors, rather than giving accurate predictions for locations where there is much data to base the prediction on. 


To analyze the issue of scale dependence, we change from indexing the individual scores by observation number to indexing them by a vector $\theta=[\mu,\sigma]$ that contains the location and scale parameters for the true predictive measure $\Q_{\theta}$ of the observations. The measure $\Q_{\theta}$ is assumed to be a location and scale transformation of a base measure $\Q$. That is, $\Q_{\theta}$ is the probability measure of the random variable
$\mu  + \sigma Z$ where $Z \sim \Q$.
	
For a given $\theta$, we let $\P_{\hat{\theta}(\theta)}$ denote the corresponding predictive distribution for the parametric model that is to be evaluated. Here $\hat{\theta}(\theta) = [\hat{\mu}(\theta),\hat{\sigma}(\theta)]$ are the location and scale parameters for the parametric model given that, the true predictive measure, $\Q$ has location and scale $\theta$. It should be noted that this is a simplification of the situation occurring for actual predictions since the location and scale of $\P_i$ in \eqref{eq:average_score} may be different for different $i$ even if the true predictive distributions $\Q_i$  have the same location and scale for all $i$. However,  it captures the important fact that the estimated location and scale typically vary with true prediction distribution location and scale. To simplify notation, we suppress the dependency on $\theta$ and simply write $\P_{\hat{\theta}}$. 
%For instance in regression if $\theta_i= \mv{X}_i\beta$ is the true mean of observation $i$, we expect  $\hat{\theta}_i= \mv{X}_i\hat{\beta}$ to be "close".
%Here it is important to note that $\Q_{\theta}$ does not represent the marginal measure of the observations, but rather the measure representing the true distribution of the predictive distribution, for instance in leave-one-out cross-validation it could be the conditional distribution of $y_i$ given $y_{-i}$.  

We assume that $\theta$ varies according to a distribution $\pi$, representing the variability of the location and scale in the scenario that is being investigated, and study the behavior of
\begin{equation}\label{eq:evaluation_function}
\tilde S(\P_{\htheta}, \Q_\theta, \pi)  =\int S \left( \P_{\htheta},\Q_\theta\right) \pi(d\theta).
\end{equation}
It is easy to see that this integral also forms a proper scoring rule given that $S$ is proper. Similar formulations of integrals over scoring rules have been used earlier in other contexts by for example \cite{Dawid1998}. 
In our case however, the integral score is used as a version of the average score where we explicitly specify the variability of the different observations through $\pi$.
Note that in this setting one can formulate the mean square error (MSE), mean absolute error (MAE) as
\begin{align*}
	&MSE = \int E_{\Q_{\theta}}\left[\left(Y-\E_{\P_{\htheta}}\left[Y \right]\right)^2\right] \pi(d\theta), 
\quad	MAE =  \int E_{\Q_{\theta}}\left[\left|Y-med(\P_{\htheta})\right|\right] \pi(d\theta).
\end{align*}
Since the functions inside the integrals are proper scoring rules they are both of type $\tilde S $. %Furthermore, the root mean squared error RMSE, defined as the square-root of the MSE, can thus be written as the square root of $\tilde S $.


In Example~\ref{ex1}, we had $\Q$ as the $\pN(0,1)$ distribution and $\pi(\theta)= \delta_{[0,0.1]}(\theta) + \delta_{[0,1]}(\theta)$. To further illustrate the idea of $\pi$, we take a spatial interpolation problem where the observation locations are generated from a Poisson processes. For a given set of locations, the observation values are simulated from a Gaussian process model with a Mat\'ern covariance function, as described in Section \ref{sec:spatstat}. A common method for model evaluation in this setup is to use a leave-one-out cross validation. Due to the spatially irregular locations, the standard deviations of the true predictive distributions for the Gaussian processes will not be identical and this is what $\pi$ is meant to capture. Although we do not get an explicit form of the distribution for the standard deviations, it is easy to simulate the process and estimate an empirical distribution. This is illustrated in Figure \ref{fig:point}. We study this problem in greater detail in Section \ref{sec:spatstat}.

\begin{figure}[t]
	\begin{center}
	\includegraphics[width=0.4\textwidth]{hist_poiss.pdf}
			\includegraphics[width=0.4\textwidth]{real_poiss.pdf}
\vspace{-0.8cm}
		\end{center}
	\caption{The distribution of the Kriging standard deviation in leave one out cross validation for a centered Gaussian random field with a Mat\'ern covariance, where the locations are generated from a Poisson point processes (left panel), and a realization of a the point pattern where the color represent the standard deviation (right panel). The points on the x-axis in the left panel correspond to the observed standard deviations in the right panel.}
	\label{fig:point}
\end{figure}

At first sight, the most natural way to remedy issues with varying scale is to require that the scoring rule is scale invariant in the sense that $S(\P_{\theta},\Q_{\theta})=S(\P_{[0,1]},\Q_{[0,1]})$. However, a scoring rule with this property is not ideal for ranking predictive distributions. The reason for this is that the scoring rule needs to disregard the sharpness of the probabilistic forecast \citet{gneiting2007probabilistic} in order to have this type of scale independence. We illustrate this problem in the following example.
	\begin{example}
		Suppose that $\mu \sim  \pN(0,1)$, and $Y \sim \pN(\mu,1)$. We want to compare two predictive measures $\P_1=  \pN(\mu,1)$ and $\P_2 = \pN(0,2)$, using $\tilde S$ with a proper scoring rule with the property $S(\Q_\theta,\Q_\theta)=S(\Q_{[0,1]},\Q_{[0,1]})$. Clearly 
		\begin{align*}
		\tilde S(\P_1,\pN(\mu,1))&=\int S(\pN(\mu,1),\pN(\mu,1)) \pi(d\mu) = \int S(\pN(0,1),\pN(0,1)) \pi(d\mu)\\
		&=S(\pN(0,1),\pN(0,1)),
		\end{align*}
		and  
		\begin{align*}
		\tilde S(\P_2,\pN(\mu,1))&=\int S(\pN(0,2),\pN(\mu,1)) \pi(d\mu) = \int \int S(\pN(0,2),  y) \pN(dy;\mu,1) \pi(d\mu) \\
		&=S(\pN(0,2),\pN(0,2)) =S(\pN(0,1),\pN(0,1)).
		\end{align*}
		Thus, although $\P_1$ is clearly a better forecast than $\P_2$,  the two forecasts cannot be separated by any scale invariant proper scoring rule.
	\end{example}
	The example shows the issue with scoring rules that do not depend on the sharpness of probabilistic forecasts. In spatial statistics one could imaging that (location and) scale invariant scoring rules will not be ideal for ranking stochastic process models with different differentiability, since the main gain for finding the correct differentiability is an improved precision rather then an improved fit of the marginal distribution. An analogue in time series analysis is to separate various degrees $p$ in AR$(p)$ processes, which will likely would be difficult using a scale invariant scoring rule. Let us emphasize that scale invariance is not necessarily a bad property of a scoring rule; however, if one uses only one scoring rule to rank predictive distributions it is. As an alternative to scale invariance, we propose the concept of local scale invariance, which requires that if one makes a small location-scale misspecification proportional to the scale of the true distribution, the difference in the scoring rule should not depend on the scale: %The following definition makes this property explicit.


\begin{Definition}\label{def:scalefunction}
	Let $S$ be a proper scoring rule and let $\Q_{\theta}=\Q_{[\mu,\sigma]}$ be a probability measure with location $\mu$ and scale $\sigma$.  Assume that there exist a constant $p\in \mathbb{R}$ and a function $s(\Q_{\theta},r):\mathcal{F} \times \mathbb{R}^2\rightarrow \mathbb{R}^+$, such that for each $r \in \mathbb{R}\times \mathbb{R}$
	$$
	S(\Q_\theta, \Q_\theta ) -  S(\Q_{\theta + t\sigma r},\Q_\theta )  = s(\Q_{\theta},r)t^{p} + o(t^{p}).
	$$	
	Then $s$ is the scale function of $S$, which is locally scale invariant if $s(\Q_{\theta},r) \equiv s(\Q,r)$. 
\end{Definition}

\begin{Remark}
If the proper scoring rule is at least twice differentiable, then $p$ equals 2.  This is due to the fact that $S$ attains it maximum at $\theta$ and hence the derivative is zero at $\theta$. Under some weak assumptions on the measure $\Q$, this is the case for all proper scoring rules studied in this article.
\end{Remark}


We will later show that the SCRPS as well as the log-score are locally scale invariant, whereas the CRPS has scale function $s(\Q_{\theta},r) =\sigma  s(\Q,r)$. To understand the effect of the scale function on the average scoring function, let us now examine what happens with misspecification in the average approximation \eqref{eq:evaluation_function}. 
	\begin{example}
Assume that we misspecify the true predictive measure $\Q_{\theta}$ by $\Q_{\theta + t\sigma r(\theta)}$, and we have two different scoring rules, both being twice differentiable, with scale functions $s_1(\Q_{\theta},r)=r^Tr$ and $s_2(\Q_{\theta},r)=\sigma r^Tr$ respectively. Plugging in the scale functions into equation \eqref{eq:evaluation_function} gives
\begin{align*}
\tilde	S_1(\Q_\theta, \Q_\theta , \pi) - \tilde S_1(\Q_{\theta + t\sigma r(\theta)},\Q_\theta ,\pi)  
&= t^2 \int r(\theta)^Tr(\theta) \pi(d\theta) +  o(t^{2}),\\
\tilde	S_2(\Q_\theta, \Q_\theta , \pi) - \tilde S_2(\Q_{\theta + t\sigma r(\theta)},\Q_\theta ,\pi)  
&= t^2 \int \sigma r(\theta)^Tr(\theta) \pi(d\theta) +  o(t^{2}).
\end{align*}
Thus scoring rule that is local scale invariant will punish misspecification proportionally to the scale, whereas the other scoring rule will put a larger penalty on misspecifications where the predictive standard deviation is large.
	\end{example}

Thus, the scale function $s(\Q_{\theta},r)$ captures the behavior seen for the normal distribution in Figure \ref{fig:bivar}, in the sense that CRPS is sensitive to the scale of the error in the observations while both SCRPS and log-score are locally scale invariant.
It is easy to see that the scale functions for the proper scoring rules defining MSE and MAE are on the form $s_{MSE}(\Q_{\theta},r) =\sigma^2  s_{MSE}(\Q,r)$ and $s_{MAE}(\Q_{\theta},r) =\sigma  s_{MAE}(\Q,r)$ repetitively. Hence, neither scoring rule is scale invariant. Note also that the scale function of the scoring rule corresponding to the root mean squared error is $\sqrt{s_{MSE}(\Q_{\theta},r)}$.


In order to ensure the existence of the scale function we need some assumptions on the probability measure $\Q_\theta$ in Definition \ref{def:scalefunction}.
The following assumptions (where the specific value of $\alpha$ varies with the scoring rule) are sufficient for the existence of the scale function for the scoring rules considered in this article. 
	\begin{Assumption}
		\label{ass1} The probability measure $\Q$ has density $q(x) = \exp(\Phi(x))$ and for $\alpha \geq 0$
		\begin{itemize}
			\item[(i)] $q(x)$ is continuously differentiable, and 
			\begin{align*}
		\E_{\Q}[\Phi'(X) ], \qquad	\E_{\Q}[ |X|^{\alpha+1} \Phi'(X) ] < \infty, \qquad
			\E_{\Q}[ |X|^{\alpha} ] < \infty. 
			\end{align*}
			\item[(ii)] $q(x)$ is twice continuously differentiable and 
			\begin{align*}
				\E_{\Q}[\Phi''(X)  ] &< \infty, \qquad
			\E_{\Q}[\left( \Phi'(X) \right)^2] < \infty, \\
			\E_{\Q}[|X|^{\alpha+3}\Phi''(X)  ] &< \infty, \qquad
			\E_{\Q}[|X|^{\alpha+3} \left( \Phi'(X) \right)^2] < \infty.
			\end{align*}
		\end{itemize}
	\end{Assumption}
	%
	It should be noted that these assumptions are far from necessary for the scoring rules considered and the corresponding scale functions thus exist for a much larger class of measures. Since our objective is  to highlight the meaning of the scale function rather than finding the largest class of measures for which it exists,  we will prove the results under these assumptions to simplify the exposition. The following result holds for the log-score.


\begin{Proposition}\label{prop:scale_ls}
	Assume that the probability measure $\Q_\theta$ satisfies Assumption \ref{ass1} for $\alpha=0$. Then the scaling function for the log-score is
	$
	s(\Q_{\theta},r)= r^TH_{\Q}r,
	$
	where $H_{\Q}$ is a $2\times 2$ matrix independent of $\theta$. Hence the log-score is locally scale invariant.
\end{Proposition}

%It be should noted that the function \eqref{eq:evaluation_function} does not take into account possible depence between the predictors and thus is not a perfect measure to compare average scoring rules when data is dependent.

\subsection{Robustness}\label{sec:robust}
Besides scale dependence, another problematic scenario is if the scoring rule is sensitive to outliers in the data. In this case, the average score \eqref{eq:average_score} may be heavily affected by only a few predictions. 
Also the sensitivity to outliers can give unintuitive results when using average scores for model selection, which is illustrated in the following example.

\begin{table}
\caption{Results for Example~\ref{ex2}.}
\centering
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{Model 1} & \multicolumn{3}{c}{Model 2}\\
& CRPS & log-score & SCRPS & CRPS & log-score & SCRPS\\
\cmidrule(r){2-4} \cmidrule(r){5-7}
$Y_1$  	& -0.0023	&  3.6862 	&   1.5351	& -0.0234 & 1.3836 & 0.3838\\
$Y_2$ 	& -4.0486 	& -16.516	& -4.9338	& -3.9204 & -14.154 & -4.5666\\
mean 	& -2.0255 	& -6.4149 	& -1.6994	& -1.9719 & -6.3853 & -2.0914\\
\bottomrule
\end{tabular}
\label{tab:ex2}
\end{table}

\begin{example}\label{ex2}
Assume that we have two competing models which are used for prediction of two variables $Y_1$ and $Y_2$. The first model (shown in black in Figure \ref{fig:bivar2}) has $\P_{\htheta_1} = \pN(0,0.01^2)$ and $\P_{\htheta_2} = \pN(5,0.8^2)$. The second model (shown in red) has $\P_{\htheta_1} = \pN(0,1)$ and $\P_{\htheta_2} = \pN(4.9,0.85^2)$. Assume that we observe $y_1 = 0$ and $y_2 = 0.5$ and compute the average CRPS, log-score, and SCRPS for each model. The results can be seen in Table~\ref{tab:ex2}.
One can note that the second model is chosen both by the CRPS and by the log-score, even though the first model is clearly more accurate for the first variable and both models are similarly inaccurate for the second. The reason for this somewhat unintuitive behavior for the CRPS is scale dependence, whereas it is caused by outlier sensitivity for the log-score. The SCRPS on the other hand chooses the first model. 
\end{example}

\begin{figure}[t]
\begin{center}
\begin{minipage}[t]{0.4\linewidth}
\begin{center}
\includegraphics[width=\textwidth]{fig2_1}
\end{center}
\end{minipage}
\begin{minipage}[t]{0.4\linewidth}
\begin{center}
\includegraphics[width=\textwidth]{fig2_2}
\end{center}
\end{minipage}
\vspace{-0.8cm}
\end{center}
\caption{Predictive distributions of two models (one shown in black and one in red) for two variables $Y_1$ (left) and $Y_2$ (right).}
\label{fig:bivar2}
\end{figure}

The apparent higher sensitivity to outliers of the log-score compared to CRPS can result in model selections where models with larger variances are favored, even though this might not be optimal for most  locations. This higher robustness of the CRPS is something that has previously been noted \citep{gneiting2007strictly}, but a natural question is if this is true also for other distributions than the normal. To assess this, we will study the behavior of $S(\P,y)$ as $|y|\rightarrow\infty$. The asymptotic rate of $S$ will in this case be a measure of the robustness of the scoring rule, and to get a scoring rule which is actually robust, we must have that $S$ remains bounded as $y$ increases. Formally, we will use the following definition of robustness of scoring rules.
\begin{Definition}
For a scoring rule $S$ on a set of probability measures $\mathcal{P}$,  and a probability measure $\P\in \mathcal{P}$, we say that $S$ has a model-sensitivity $\alpha_\P$ if $S(\P,y)\sim |y|^{\alpha_\P}$  as $|y|\rightarrow\infty$. The sensitivity index of the scoring rule is defined as $\alpha = \sup_{\P\in\mathcal{P}} \alpha_\P$. The scoring rule is robust if $\alpha=0$.
\end{Definition}

In the case of the log-score and the normal distribution, we see that the model-sensitivity is $\alpha_\P=2$, so the log-score is not robust. Using the expression of the CRPS for the normal distribution from Appendix \ref{app:gauss}, we get that the model-sensitivity in this case is $\alpha_\P=1$. Thus, the CRPS has a lower sensitivity than the log-score in the Gaussian case, but it is not robust. In fact, it is not always the case that the model-sensitivity is lower for the CRPS compared to the log-score. A simple counter example to this is to take $\P$ as the Laplace distribution, with $\log f(y) \sim y$ and $CRPS(\P,y)\sim y$ as $y\rightarrow\infty$.



\section{Kernel scores and robustness}\label{sec:kernel_scores}

The CRPS is a special case of the larger class of kernel scores, coined by \cite{dawid2007geometry}, which are created using a negative definite kernel. A real-valued function $g$ on $\Omega \times \Omega$, where $\Omega$ is a non-empty set, is said to be a negative definite kernel if it is symmetric in its arguments and if $\sum_{i=1}^n\sum_{j=1}^n a_i a_j g(x_i,x_j) \leq 0$ for all positive integers $n$, all $a_1,\ldots,a_n \in \mathbb{R}$ such that $\sum_{i=1}^n a_i=0$, and all $x_1,\ldots,x_n \in \Omega$. 
%
Given a negative definite kernel, the kernel score is created as in the following theorem by \cite{gneiting2007strictly}. 

\begin{Theorem}[\cite{gneiting2007strictly}]\label{thm:kernel}
Let $\P$ be a Borel probability measure on a Hausdorff space $\Omega$. Assume that $g$ is a non-negative, continuous negative definite kernel on $\Omega \times \Omega$ and let $\mathcal{P}$ denote the class of Borel probability measures on $\Omega$ such that  $\E_{\P,\P}\left[ g(X,Y) \right] < \infty$. Then the scoring rule
\begin{equation}\label{eq:kernel_score}
\Sker_g(\P, y) := \frac{1}{2} \E_{\P,\P} \left[g(X,Y) \right] - \E_{\P} \left[g(X,y) \right]
\end{equation}
is proper on $\mathcal{P}$. 
\end{Theorem}

One example of a family of negative definite kernels that can be used in the theorem is $g_{\alpha}(x,y) = |x-y|^{\alpha}$ for $\alpha\in (0,2]$, and we introduce the shorthand notation $\Sker_{\alpha}(\P,y)$ for this choice. The CRPS is the special case $\Sker_1(\P,y)$.

We are now interested in whether the kernel scores satisfy our desired properties of scale invariance and robustness. Regarding robustness, the property is highly dependent on which kernel that is used. 
Specifically, we have the following theorem.

\begin{Theorem}
	\label{the:kernelrob}
	Let $\P$ be a Borel probability measure on a normed space $\Omega$, with norm $||\cdot||$.
	  Assume that	 $g$ is a non-negative, continuous negative definite kernel on $\Omega \times \Omega$, such that  $g(x,y)=g_0(||x-y||)$, with $g_0(x) \sim |x|^\alpha$ for some $\alpha>0$, and $\E_{\P}[g_0(||X||)] < \infty$. Then $S^{ker}_g(\P,y) \sim -||y||^\alpha.$
\end{Theorem}
The theorem shows that $\Sker_{\alpha}$ is not a robust scoring rule. However, we may modify the kernel in order to make it robust. For example:%An example of a robust scoring rule is given in the following corollary. 

\begin{Corollary}
Let $\P$ be a Borel probability measure on $ \mathbb{R}$, and for $c>0$ define
\begin{equation}\label{eq:truncated_kernel}
g_c(x,y) = \begin{cases}
|x-y| & |x-y|<c,\\
c & \mbox{otherwise.}
\end{cases}
\end{equation}
Then the \textbf{robust CRPS} (rCRPS) defined as $\Sker_{1,c}(\P, y) := \Sker_{g_c}(\P, y)$ is a proper scoring rule on the class of Borel probability measures on $ \mathbb{R}$.
\end{Corollary}
\begin{proof}
The function $g_c$ is negative definite since $g_c(x,y) = 1 - r(x,y)$ where $r$ is the triangular correlation function. The result therefore follows from Theorem~\ref{thm:kernel} since $\pE_{\P,\P}[g_c(X,X)]\leq c$. \qed
\end{proof}

The reason for the name of the scoring rule is that it can be viewed as a robust version of the CRPS, where the constant $c$ defines a limit where deviations are not further punished. Analytic expressions for this score in the case of the Gaussian distribution are given in Appendix~\ref{app:gauss}. Naturally, many other robust scoring rules can be constructed by replacing the triangular correlation function with some other compactly supported correlation function. 

The next questions is whether the kernel scores, robust or not, are scale invariant. The following proposition shows that  $S^{ker}_{\alpha}$ is scale dependent.

\begin{Proposition}\label{prop:kernel_scale}
	Let $\alpha \in (0,2]$ and assume that $\Q$ is a probability measure satisfying Assumption~\ref{ass1}. 
	 Then $S^{ker}_{\alpha}$ has scale function 
$$s(\Q_{\theta},r)=\sigma^{\alpha}s(\Q,r) = \sigma^{\alpha}r ^T\E_{\Q,\Q}[H^{\alpha}_{\Q}(X,Y)]r$$
where $H^{\alpha}_{\Q}(X,Y)$ is a $2\times 2$ matrix independent of $\theta$.
\end{Proposition}
In order to make the scoring rule locally scale invariant one would have to scale it with $\sigma$, which in reality almost never is available a priori to the forecaster. %However $\sigma$ is a simplification and in reality the scaling of the observation will depend on many different sources and will almost never be 
For the robust CRPS we have the following result.
\begin{Proposition}\label{prop:scale_rob}
	Let $\Q$ be a probability measure satisfying Assumption \ref{ass1} for $\alpha=1$. Then $S^{ker}_{1,c}$ has scale function
	$$s(\Q_{\theta},r)=\sigma r^T\E_{\Q,\Q}\left[ H_{\Q}(X,Y)\mathbb{I}\left(\left|X-Y\right|<\frac{c}{\sigma}\right)\right]r,$$
where $H_{\Q}(X,Y)$ is a $2\times 2$ matrix independent of $\theta$.
\end{Proposition}

This result implies that when applying $S^{ker}_{1,c}$ in a situation with varying $\sigma$, one puts lower weights on the larger values of $\sigma$ since $c$ is fixed. Thus the robustness is with respect to  the marginal data predictive measure, $\int \Q_{\theta} \pi(d\theta)$, and not with respect to the predictive measure, $\Q_{\theta}$. This means that the robustness will protect against outliers that are large on an absolute scale of the predictive measure. On the other hand, the robustness cannot protect against outliers for predictions that are relatively certain and have  small $\sigma$.
%

In order to make the scoring rule robust against outliers of $\Q_{\theta}$ the bound would need to be scaled with $\sigma$, which as mentioned above is unknown a priori. It is to the authors' knowledge an open question how to create a proper scoring rule that protects against outliers in $\Q_{\theta}$. One option that could work in practice is to set $c$ dependent on some reference predictive distribution. Since $c$ should only protect against outliers it does not seems as invasive as scaling the actual scoring rule with a reference score, but is nevertheless still problematic. 


\section{$h$-function proper kernel scoring rules}\label{sec:standardized_scores}
In the previous section, we saw that one could make the kernel scores robust by adjusting the kernel, but that they in general are scale dependent. Because of this, we now want to construct a new family of scoring rules which can be made scale independent. This is done in the following theorem.

\begin{Theorem}\label{thm:convexkernel}
Let $\Omega$ be a Hausdorff space and let $\P$ be a Borel probability measure on $\Omega$. 
Assume that $g$ is a non-negative, continuous negative definite kernel on $\Omega \times \Omega$ and that $h$ is a monotonically decreasing convex differentiable function on $\mathbb{R}^+$.  Then the scoring rule
	\begin{equation}\label{eq:scaled_score}
		S^h_g(\P, y) := h\left(\E_{\P,\P}\left[g(X,Y)\right]\right)  +  2h'\left(\E_{\P,\P}\left[g(X,Y)\right]\right) \left(\E_{\P}\left[g(X,y)\right] - \E_{\P,\P}\left[g(X,Y)\right] \right)  
	\end{equation}
	is proper on the class of Borel probability measures on $\Omega$ such that $\E_{\P,\P}\left[ g(X,Y) \right] < \infty$.
\end{Theorem}

It should be noted that the idea of the theorem is similar to the construction of the supporting hyperplane in \cite[p.22]{Dawid1998}. Furthermore, the theorem could be generalized slightly by not requiring that $g$ is a continuous negative definite kernel but rather a function satisfying $g(x,y)\leq \frac12 \left(g(x,x) + g(y,y)\right)$. 

With $g(x,y)=|x-y|$ and $h(x)=-\frac{1}{2} x$, $S^h_g$ is the regular CRPS. This scoring rule thus has the least convex (as it both convex and concave) $h$ possible which therefore is (up to a scaling factor) the fastest declining $h$ possible. %Another interesting example is $h(x)=-\frac{1}{2} \log(x)$ and $g(X,Y)=(X-Y)^2$ which results in a proper scoring rule that is very similar to the log-score.
With $h(x) = -\frac{1}{2} \log(x)$, the proper scoring rule is given by
$$
S^{-\frac{1}{2} \log(x)}_g(\P, y) = -\frac{1}{2}\log(\E_{\P,\P}[g(X,Y)]) - \frac{\E_{\P}[g(X,y)]}{\E_{\P,\P}[g(X,Y)]} +1.
$$
Due to the second term in this expression, we will refer to it as the standardized kernel scoring rule with kernel $g$.

There are of course a myriad of options that can be used as $h$. Two interesting options are $h(x)=-\sqrt{x}$ and $h(x)=-x^2$, where the former should act similarly to the standardized kernel score whereas the latter will have a strong punishment of large uncertainty. 

This flexibility is important since it allows for a wide range of generalized entropy terms, which correspond to different penalties for a priori uncertainty, while remaining proper scoring rules. This is discussed further in Appendix \ref{sec:entropy}.

As for the usual kernel scores, $g_{\alpha}(x,y) = |x-y|^{\alpha}$ for $\alpha\in (0,2]$ is a natural choice of kernel, and we introduce the shorthand notation $\Ssker_{\alpha}(\P,y) = \Ssker_{g_\alpha}(\P,y)$ for the corresponding standardized kernel scoring rule. The special case $\Ssker_{1}(\P,y)$ in \eqref{eq:scrps} is interesting since it provides a standardized analogue to the CRPS. Note also that \begin{align*}
	\Ssker_2(\P,y) &= 
	-\frac{1}{2}\log(\E_{\P,\P}[(X-Y)^2]) - \frac{\E_{\P}[(X-y)^2]}{\E_{\P,\P}[(X-Y)^2]} +1 \\
	&=
	-\frac{\left(y-\E_{\P}\left[Y\right]\right)^2}{\V_{\P}\left[Y\right]} - \frac{1}{2} \log\left(\V_{\P}\left[Y\right] \right),
	\end{align*}
which is the Dawid-Sebastiani score.
%
The following proposition shows the local scale invariance for $\Ssker_{\alpha}$. 

\begin{Proposition}
	\label{prop:scale_stand}
	Let $\alpha \in (0,2]$ and assume that $\Q$ is a probability measure satisfying Assumption \ref{ass1}. Then
	 the standardized proper kernel scoring rule $\Ssker_{\alpha}$ has scale function
$s(\Q_{\theta},r)=r^T\E_{\Q,\Q}[H_{\Q}^{\alpha}(X,Y)]r$, where $H^{\alpha}_{\Q}(X,Y)$ is a $2\times 2$ matrix independent of $\theta$.
\end{Proposition}

Thus $\Ssker_{\alpha}$ is scale independent for $\alpha \in (0,2]$.
 The robustness of the standardized kernel scores is clearly equal to that of the corresponding kernel score, and thus depends on the kernel. Therefore, $\Ssker_{\alpha}$ has the same robustness properties as $\Sker_{\alpha}$:% We formulate this as a theorem.
\begin{Theorem}\label{thm:sta_rob}
Let $\P$ be a Borel probability measure on a normed space $\Omega$, with norm $||\cdot||$.
	  Assume that	 $g$ is a non-negative, continuous negative definite kernel on $\Omega \times \Omega$, such that  $g(x,y)=g_0(||x-y||)$, with $g_0(x) \sim |x|^\alpha$ for some $\alpha>0$, and $\E_{\P}[g_0(X)] < \infty$. 
	  Then $\Ssker_{g}(y,\P) \sim -\|y\|^\alpha.$
\end{Theorem}


Another interesting scoring rule is the standardized kernel score which uses the kernel \eqref{eq:truncated_kernel}, which we denote as rSCRPS or $\Ssker_{1,c}$, where $c$ is the constant in the function $g_c$. It could be thought of as a robust version of the SCRPS, but it should be noted that it cannot be scale independent by the same reasons as for the rCRPS. We will however later use this in one of the applications as an option that protects against outliers but has better scaling properties than the CRPS.

 
So far, we have only considered how to formulate scale invariant versions of kernel scores. However, there exists several other popular scoring rules which are not defined through kernels like the CRPS. Examples of such scores are the continuous ranked logarithmic score \citep{juutilainen2012exceedance,todter2012generalization} and the threshold-weighted continuous ranked probability score \cite{gneiting2011comparing,Lerch2016}. It is not clear whether they are scale invariant, and Theorem~\ref{thm:convexkernel} cannot be directly used to create a standardized version. However, in those cases, the following theorem can instead be used. The theorem defines a transformation of a negative proper scoring rule, that is still a proper scoring rule and which, at least intuitively, should be less scale dependent.
\begin{Theorem}\label{thm:general_scale}
Let $S(\P,y)$ be a negative oriented proper scoring rule on a set of probability measures $\mathcal{P}$, then
\begin{align*}
	\Strans_S(\P,y) := \frac{S(\P,y)}{|S(\P,\P)|} -  \log(|S(\P,\P)|)
\end{align*}
is also a proper scoring rule on $\mathcal{P}$.
\end{Theorem}

One can note here that if one applies the theorem on the CRPS, the result is two times the SCRPS defined in \eqref{eq:scrps}. This serves as another motivation for why the SCRPS can be seen as a standardized version of the CRPS.


\section{Applications}\label{sec:application}
%In this section, we illustrate the previous findings in three different applications. 

\subsection{A stochastic volatility model}
Here we want to highlight the difference between scaled and non-scaled scoring rules when there is variability in the scaling of the data which is caused by the model. Consider the following stochastic volatility model \citep{shephard1994partial},
\begin{align*}
X_t &= a X_{t-1} + \epsilon^X_t, \quad t = 1, 2,\ldots, \\
y_t &= \epsilon_t^Y \exp(X_t),
\end{align*}
where $\epsilon^X_t \sim \pN(0,\sigma^2_X)$ and $\epsilon^Y_t \sim \pN(0,\sigma^2_Y)$.  Throughout this example, we let $a=0.95$, $\sigma_Y=1$, and $\sigma_X=0.5$. Figure \ref{fig:SimVol} displays realizations of $Y_t$ and $X_t$. 

\begin{figure}[t]
	\centering
\includegraphics[scale=0.35]{x_Vol.pdf}
\includegraphics[scale=0.35]{y_Vol.pdf}
\caption{A realization of the volatility $x$ (left), and the observation of the model $y$ (right).}
\label{fig:SimVol}
\end{figure}


Although the observations are equally spaced, the varying volatility will result in that the proper scoring rules will weight the observation differently. We explore the model under a simplified assumption that we observe $X_t$ and wants to predict $y_t$, which simplifies the analysis without altering the message that we want to convey through the application.
 
 
 To see how the stochastic volatility affects model selection, we compare how often the average score for each scoring rule is higher for the correct model compared to models with misspecified $\sigma_Y$. We simulate $500$ different realizations of the volatility model, where each simulation is a time series of length $600$. Figure \ref{fig:SelectVol} shows the percentage out of these realizations where the correct model, with $\hat{\sigma}_Y=\sigma_Y$, is chosen (has the largest mean score) for the three different scoring rules. As alternative models in the comparison, one with $\hat{\sigma}_Y = \sigma_Y+ \Delta$ and one with $\hat{\sigma}_Y = \sigma_Y - \Delta$ are used. The figure shows the result as a function of $\Delta \in (0,0.5)$. We can note that the SCRPS and the log score are virtually identical whereas CRPS preforms considerably worse.
 
 Further comparisons of the scoring rules for this example can be seen in Appendix~\ref{sec:entropy}.
 % and standardized kernel score with absolute kernel. In Figure \ref{fig:scoringRuleVol}, we show the resulting scoring rule value, the calibration score and the sharpness score as a function of the one step ahead predicted volatility. We see that both scoring rules are effected by the expected volaility. However unlike CRPS the effect for sCRPS comes only from the sharpness of the scoring rule. For the CRPS we see clearly the linear term in the sharpness and for sCRPS we see the logarithmic term. The calibration term for sCRPS is seemingly unfected by the volatility, wheras the variability of the calibration value increases with an increasing volatility.

\begin{figure}
	\centering
	\includegraphics[scale=0.7]{vol_modelselect.pdf}
	\caption{Probability of selecting the true model, $\hat{\sigma}_Y=\sigma_Y=1$, compared to the model with $\hat{\sigma}_Y = \sigma_Y \pm \Delta $, for the three different scoring rules.}
	\label{fig:SelectVol}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\linewidth]{field_simulation}
\includegraphics[width=0.39\linewidth]{field_locations}
\caption{Gaussian random field simulation and observation locations.}
	\label{fig:spatial_sim}
\end{figure}
\subsection{An application from spatial statistics}
\label{sec:spatstat}
A common use of proper scoring rules is to evaluate the predictive power of random field models in spatial statistics. As an illustration of this application, we generate $n=100$ observations $y_i = X(\mv{s}_i), i=1,\ldots, n$ of a mean zero Gaussian random field with a Mat\'ern covariance function 
$$
C(h;\mv{\Psi}) = \frac{\sigma^2}{2^{\nu-1}\Gamma(\nu)} (\kappa h)^{\nu} K_{\nu}(\kappa h).
$$
Here $\mv{\Psi} = (\kappa,\sigma,\nu)$ is a vector with the parameters of the model which we choose as $(50, 1, 3)$ so that the field has variance $1$ and a practical correlation range of approximately $0.1$. A simulation of the model is shown in Figure~\ref{fig:spatial_sim}, which also shows an example of the observation locations $\mv{s}_i$ drawn at random from a uniform distribution on $[0,1]\times [0, 1]$. 

A measure of the predictive quality of a model with parameters $\mv{\Psi}^*$ is the average score \eqref{eq:average_score} in a cross-validation scenario. That is, $\P_{i} = \pN(\mu_i(\mv{\Psi}^*), \sigma_i(\mv{\Psi}^*)^2)$ is the conditional distribution of $X_i$ given given all data except that at location $\mv{s}_i$, which we denote by $\mv{y}_{-i}$. If we let $\mv{\Sigma}$ denote the covariance matrix of $y_{i}$, and let $\mv{c}$ be a vector with elements $ \mv{c}_j = C(\|s_i - s_j\|;\mv{\Psi}^*)$, the parameters of the predictive distribution are $\mu_i(\mv{\Psi}^*) = \mv{c}^T \mv{\Sigma}^{-1}\mv{y}_{-i}$ and $\sigma_i(\mv{\Psi}^*)^2 = \sigma^2 - \mv{c}^T \mv{\Sigma}_i^{-1}\mv{c}$.

One can note that $\sigma_i(\mv{\Psi}^*)^2$ depends on the spatial configuration of the observation locations, where prediction locations close to observation locations will have lower variances.% Thus, if one were to plot the individual scores against the smallest distance between the prediction location and the other observation locations, a similar behavior as in Figure \ref{fig:scoringRuleVol} would be observed. %This means that, even though the model for $X$ is stationary, the importance of each observation $y_i$ for the average score will vary if the scoring rule is scale dependent, and observations far away from other observations will in general be the most important for the average score. 

Scale dependence of scoring rules increases the variance of the values for large distances, which in turn may result in a larger variance of the average score. That the average CRPS has a larger variance than the average SCRPS means that it could be more likely that $S_n(\mv{\Psi}) < S_n(\mv{\Psi}^*)$ even if the data is generated using the parameters $\mv{\Psi}$. That is, it is more likely that the incorrect model choice is made if the average score is used for model selection. This is illustrated in the top left panel of Figure~\ref{fig:spatialKappa}, which shows the proportion of times that $S_n(\mv{\Psi}) > S_n(\mv{\Psi}^*)$ as a function of $\Delta$ when $\mv{\Psi}^* = (\kappa\pm \Delta, \sigma, \nu)$ and $n=100$ observations is generated using $\mv{\Psi} = (\kappa, \sigma, \nu) = (50, 1, 3)$. The top right panel shows the same result with $n=200$ observations. In both cases, the results are shown for CRPS, SCRPS, and log-score, as well as the robust versions of CRPS and SCRPS with a limit value $c=2$. This limit value is equal to two times the variance of the field and is thus a quite high value given that the predictive variances often will be much lower than this. The limit should therefore not affect the predictions except at the locations close to potential outliers. 
%
 One can note that, compared to CRPS and the robust CRPS, the log-score, SCRPS, and the robust SCRPS more often make the correct model choice for a given value of $\Delta$. One can also note that the robust scores in this case perform similarly to the regular scores, since the value of $c$ is rather high and since there are no outliers in the data. The results are based on $2000$ different simulations of the field $X$ and the observation locations when $n=100$ and on $1000$ simulations when $n=200$. 

To illustrate why the robust scores may be useful, we redo the same simulation study with only one difference: For one of the observations $y_i$, chosen at random, we add a $\pN(0,5^2)$ variable, which thus makes this observation an outlier that does not follow the assumed model. The lower row of Figure~\ref{fig:spatialKappa} shows the results. One can note that the outlier makes it more likely to choose incorrect model, but that this effect is reduced if the robust scores are used. 
In summary, if one were to choose one scoring rule to use for this type of data, where outlier may be present, the robust SCRPS is likely a good choice since it performs well both with and without outliers. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.4\linewidth]{spatial_kappa_n100}
\includegraphics[width=0.4\linewidth]{spatial_kappa_n200}
\includegraphics[width=0.4\linewidth]{spatial_kappa_n100_outlier}
\includegraphics[width=0.4\linewidth]{spatial_kappa_n200_outlier}
\caption{Probability of selecting the true spatial model with $\kappa = 50$ instead of the models with $\kappa = 50 \pm \Delta$ for five different scoring rules. The results are based on $n= 100$ observations and $2000$ simulations to the left, and $n = 200$ observations and $1000$ simulations to the right. In the top row, the data does not have any outliers, whereas it has one outlier in the bottom row. }
	\label{fig:spatialKappa}
\end{figure}

\subsection{Negative binomial regression}

As a final application, we consider a negative-binomial regression model from an application in Space Syntax research \citep{hillier1993}. The application is described in detail in \citep{spacesyntax2019}. The data we consider consist of daily counts of the number of pedestrians that walked on 227 different street segments in Stockholm, Sweden. The data can be explored in the web application available at  \url{http://129.16.20.138:3838/stepflow/stepflow/}, and we refer to   \citep{spacesyntax2019} and \citep{Pont2019a} for details about how the data was collected.
%
The goal is to explain the number of pedestrians walking on a given street through covariates in a regression model. If such a model fits well, it could for example be used to predict the number of pedestrians in new neighborhoods that are planned to be built in the city. Since the observations are counts, a reasonable model is a negative-binomial regression model. We assume that the observed count at street segment $i$ has a negative binomial distribution, $Y_i \sim \mbox{nBin}(\mu_i, s)$, where $\mu_i$ is the expected value of $Y_i$ and $s>0$ is a dispersion parameter that controls the variance of $Y_i$, which is $\pV(Y_i) = \mu_i + \mu_i^2/s$.  The mean is modeled as 
\begin{equation}\label{eq:regression}
\log(\mu_i) = \sum_{k=1}^K \theta_k X_{k,i},
\end{equation}
where $X_{k,i}$ is the value of the $k$th covariate at street segment $i$, and $\theta_k$ is the corresponding regression coefficient. We have ten covariates: 1) The weekday the measurement was taken; 2) The number of schools within 500m walking distance to the street segment;  The number of public transport nodes 3)  on the street segment, and 4) within 500m walking distance to the street segment; the number of local markets such as shops and caf\'es 5) on the street segment, and 6) within 500m walking distance to the street segment; as well as three covariates that related to the centrality of the street in the street network as well as the density of the buildings around the street \citep[see][for further details]{spacesyntax2019,Pont2019a}. 

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{pedestrian_crps}
\caption{Negatively oriented CRPS and SCRPS plotted against scaled residuals. The size and color of the points are determined by the expected value of the predictor.}
	\label{fig:pedestrian}
\end{figure}

We fit the model, to the data, using the R function \texttt{glm.nb} function from the MASS package \citep{MASSpackage}, and compute the CRPS and SCRPS value for each observation based on the model. In Figure \ref{fig:pedestrian}, the values of the scoring rules for each observation are plotted against the scaled residuals for the observations, defined as
$$
e_i = \frac{|y_i - \hat{\mu}_i|}{\hat{\sigma}_i} = \frac{|y_i - \hat{\mu}_i|}{\sqrt{\hat{\mu}_i+\hat{\mu}_i^2/\hat{s}}},
$$
where $\hat{s}$ is the estimated dispersion parameter and $\hat{\mu}_i$ is given by \eqref{eq:regression} with the estimated regression parameters. In the figure, the size and color of each observation is determined by $\hat{\mu}_i$, and one can note that the large CRPS values do not coincide with the observations that have large standardized residuals. Instead the magnitude of the CRPS values is mainly determined by $\mu_i$. This is a clear example of scale dependence, where the values for streets with high expected counts will be much more important than streets with low counts for the average CRPS. 
It should be noted here that the two previous applications had Gaussian predictive distributions, which were uniquely specified by scale and location parameters. This is not the case for the negative-binomial distribution, since it does not have scale and location parameters. Nevertheless, we see that the scaling issue remains the same, and that average SCRPS gives much more reasonable result compared to average CRPS.


Obviously one should be very careful with using average scores in this case, since a single observation might drastically change the average score. To illustrate this, we compute the average CRPS of the $k$ observations with smallest values of $\mu_i$ and divide this number for each $k$ by the average CRPS for all observations.  The result is shown as a function of $k$ in Figure \ref{fig:pedestrian2}, where we also show the same thing for the SCRPS. One can note that removing around 20 of the observations with the largest values of $\mu_i$ reduces the average CRPS by a half, whereas the SCRPS is much less sensitive to the removal of observations. 



\begin{figure}[t]
\centering
\includegraphics[width=0.6\linewidth]{pedestrian_change}
\caption{The average score of the $k$ smallest observations divided by the average score of all observations.}
	\label{fig:pedestrian2}
\end{figure}



\section{Discussion}\label{sec:discussion}
The main take-away message of this work is that one should  be careful with using averages of scoring rule values for model selection in cases when the observations and the predictive distributions have varying scale. To analyze and describe the issue mathematically, we introduced the concept of scale dependence for scoring rules. It was shown that the popular scoring rules CRPS, RMSE, and MAE are scale dependent and that this may lead to unintuitive model choices. 

To address this issue we introduced a new class of scoring rules, the $h$-function proper kernel scores, which has as special cases the CRPS as well as the SCRPS, that can be viewed as a scale invariant version of the CRPS. We also introduced the concept of robustness of scoring rules and showed how one can define robust $h$-function proper scoring rules, where we in particular defined a robust version of the CRPS.  An important property of the $h$-function proper kernel scores is that they are as easy to compute as the CRPS, and that they can be approximated using Monte Carlo integration in the same way as CRPS for more complicated models where there are no analytic expressions for the scoring rules. 
%
In the three applications we demonstrated that SCRPS gives more reasonable scores compared to CRPS because of the scale invariance.

An important issue that we have not addressed is that there is typically dependence between the predicted observations that are used in the average. How to take this dependence into account when comparing models is an interesting topic for future research, and we believe that scale dependence will be an important issue to consider also in that scenario. 
%In our opinion it is seems unlikely that scaling issue will not remain an important property there also.

%An advantage with the regular CRPS is that it allows for comparison with deterministic prediction models. This is not possible for the introduced SCRPS since any incorrect prediction with zero uncertainty would get an infinite score. An alternative scoring rule that allows for such comparisons is use $h(x)=-\frac{1}{2}\log(x+c)$ for $c>0$ as $h$-function. The result of the scoring rule will then depended on the choice of the truncation parameter $c$ which need to be set by the user, and we leave investigations of how to best do that for future research. 




